Predict-and-Critic: Accelerated End-to-End Predictive Control for Cloud Computing through Reinforcement Learning

Cloud computing holds the promise of reduced costs through economies of scale. To realize this promise, cloud computing vendors typically solve sequential resource allocation problems, where customer workloads are packed on shared hardware. Virtual machines (VM) form the foundation of modern cloud computing as they help logically abstract user compute from shared physical infrastructure. Traditionally, VM packing problems are solved by predicting demand, followed by a Model Predictive Control (MPC) optimization over a future horizon. We introduce an approximate formulation of an industrial VM packing problem as an MILP with soft-constraints parameterized by the predictions. Recently, predict-and-optimize (PnO) was proposed for end-to-end training of prediction models by back-propagating the cost of decisions through the optimization problem. But, PnO is unable to scale to the large prediction horizons prevalent in cloud computing. To tackle this issue, we propose the Predict-and-Critic (PnC) framework that outperforms PnO with just a two-step horizon by leveraging reinforcement learning. PnC jointly trains a prediction model and a terminal Q function that approximates cost-to-go over a long horizon, by back-propagating the cost of decisions through the optimization problem \emph{and from the future}. The terminal Q function allows us to solve a much smaller two-step horizon optimization problem than the multi-step horizon necessary in PnO. We evaluate PnO and the PnC framework on two datasets, three workloads, and with disturbances not modeled in the optimization problem. We find that PnC significantly improves decision quality over PnO, even when the optimization problem is not a perfect representation of reality. We also find that hardening the soft constraints of the MILP and back-propagating through the constraints improves decision quality for both PnO and PnC.

==> MILP.tex <==
\subsection{MILP Formulation}
The objective of the CLOUD packing problem is to minimize the sum of costs incurred by new hosts, migrations and throttling. We assume that there are a maximum of $N$ VMs at any time in a prediction horizon of $T$ steps. Each host has a maximum capacity $C$. The decision variables are described below.
\begin{align*}
    \text{alloc}_{iht} &= \begin{cases} \text{resources allocated to VM i}\\\;\;\;\;\;\text{(if assigned to host h) at time t} \end{cases} \\
    \text{used}_{ht} &= \begin{cases} 1, \text{ if host h is used at time t} \\ 0, \text{ otherwise} \end{cases}\\
    \text{placed}_{iht} &= \begin{cases} 1, \text{ if VM i is assigned to host h at time t} \\ 0, \text{ otherwise} \end{cases}\\
    \text{migr}_{iht} &= \begin{cases} 1, \text{ if host h is migrating VM i at time t} \\ 0, \text{ otherwise} \end{cases}\\
    \text{throt}_{it} &= \begin{cases} \text{throttling fraction given as } \frac{1}{C} (\text{demand minus} \\\text{resources allocated to VM i at time t}) \end{cases}
\end{align*}
In the objective, the cost of hosts and migrations is proportional to the the number of hosts and migrations respectively. The cost of a throttled VM increases with the fraction of demand that is unmet ($th_{it}$). The objective is formulated as follows for a horizon $T$.
\begin{align*}
    \min \; \sum_{t=1}^{T} \left( h_{\$} \; n_{hosts} + m_{\$} \; n_{migrations} + th_{\$} \;f_{throttled} \right)
\end{align*}
where $n_{hosts}$ is the number of hosts, $n_{migrations}$ is the number of migrations, $f_{throttled}$ is the fraction of unmet demand, $h_{\$}$ is the real cost of spinning up one host, $m_{\$}$ is the cost of one migration, and $th_{\$}$ is the real cost associated with throttling 1 resource unit.

It can be written as a linear function of the decision variables as below.
{ \small \begin{align}
    \min \; \sum_{t=1}^{T} \Bigg( h_{\$} \sum_{h=1}^{N} \text{used}_{ht}& + \frac{m_{\$}}{2} \sum_{h=1}^{N} \sum_{i=1}^{N}  \text{migr}_{iht} \nonumber \\
    &+ th_{\$} \sum_{i=1}^N \text{throt}_{it}\Bigg) \label{obj}
\end{align} }
The constraints of the problem are given below. Initially, we have the domains of all the decision variables.
{ \small \begin{align}
    \text{alloc}_{iht} &\in \Z^{+} \;\;\;\;\;\;\; \forall \; i, \forall \; h, \forall \; t \label{c0iv}\\
    \text{used}_{ht} &\in \{0, 1\}\;\;\;\;\;\;\; \forall \; h, \forall \; t \label{c0i}\\
    \text{placed}_{iht} &\in \{0, 1\}\;\;\;\;\;\;\; \forall \; i, \forall \; h, \forall \; t \label{c0ii}\\
    \text{migr}_{iht} &\in \{0, 1\}\;\;\;\;\;\;\; \forall \; i, \forall \; h, \forall \; t \label{c0iii}\\
    \text{throt}_{it} &\in \R\;\;\;\;\;\;\; \forall \; i, \forall \; t \label{c0v}
\end{align} }
First, we have that the sum of resources allocated to VMs on each host should be less than or equal to the hosts capacity if it is in use.
{ \small \begin{align}
    \sum_{i=1}^N \text{alloc}_{iht} \leq C \; \text{used}_{ht} \;\;\;\;\;\;\; \forall \; h , \forall \; t \label{c1}
\end{align} }
Second, we have that each VM should only be on one host.
{ \small \begin{align}
    \;\;\;\; \sum_{h=1}^N \text{placed}_{iht} = 1 \;\;\;\;\;\;\; \forall \; i, \forall \; t \label{c2}
\end{align} }
Third, an VM should only be placed on a host if it was allocated non-zero resources on that host.
{ \small \begin{align}
    \text{placed}_{iht} \geq \frac{\text{alloc}_{iht}}{C}  \;\;\;\;\;\;\; \forall \; i, \forall \; h, \forall \; t \label{c3}
\end{align} }
Fourth, we set the throttling fraction as the difference in demand and actual resource allocation divided by the capacity of the host. We denote the demand of VM $i$ at time $t$ with $y_{it}$.
{ \small \begin{align}
    \text{throt}_{it} = \frac{\left(y_{i(t+1)} - \sum_{h=1}^N \text{alloc}_{iht} \right)}{C} \;\;\;\;\;\;\; \forall \; i, \forall \; t\label{c4}
\end{align} }
In practice, we move this term to the objective. We can drop the demand term as it is does not depend on any decision variables.

Fifth, we add migration constraints. Namely, the number of migrations involving any host should be less than or equal to $Max\_migrs$, and that $\text{migr}_{iht} = |\text{placed}_{iht} - \text{placed}_{ih(t+1)}|$.
{ \small \begin{align}
    \sum_{i=1}^N \text{migr}_{iht} &\leq Max\_migrs \;\;\; \forall \; h, \forall \; t \label{c7i}\\
    \text{placed}_{iht} - \text{placed}_{ih(t+1)} &\leq \text{migr}_{iht} \;\;\;\;\; \forall i, \forall h, \forall t \label{c7ii}\\
    \text{placed}_{iht} - \text{placed}_{ih(t+1)} &\geq - \text{migr}_{iht} \;\;\;\;\; \forall i, \forall h, \forall t \label{c7iii}
\end{align} }
where we set $Max\_migrs$ to 1. To improve speed of solution computation with MILP solvers, we add the following constraints to reduce the size of the enumeration tree for the ILP solver without affecting the generality of the formulation. The first constraint ensures that hosts are used in increasing order (i.e. host 1 is utilized before host 2 when both are empty). The second constraint above ensures that VM 1 is packed in host 1, VM 2 in either hosts 1 or 2, VM 3 in either hosts 1, 2, or 3 and so on.
{ \small \begin{align}
    \text{used}_{ht} &\geq \text{used}_{(h+1)t}  \;\;\;\;\;\;\; \forall \; h, \forall \; t \label{c8i}\\
    \text{placed}_{iht} &= 0 \;\;\;\;\;\;\; \forall \; i, \forall \; h > i, \forall \; t \label{c8ii}
\end{align} }
Thus, our MILP is given by objective \ref{obj} with constraints \ref{c0i} -- \ref{c8ii}. We call this the \textbf{primary MILP}.

Additionally, we include a soft constraint that states that an VM $i$ (on any host $h$) at time $t$ can only be allocated an amount less than or equal to its upcoming demand ($y_{i(t+1)}$). This accounts for an internal hueristic in the simulator that does not allow allocations larger than the actual demand at the next step. The constraint is given as follows.
{ \small \begin{align}
    \;\;\;\; \text{alloc}_{iht} \leq y_{i(t+1)} \; \text{placed}_{iht} \;\;\;\;\;\;\; \forall \; i, \forall \; h, \forall \; t  \label{c4b}
\end{align} }


As a soft constraint, inequality \ref{c4b} is added to the objective as follows.
{ \small \begin{align}
    &\min \; \sum_{t=1}^{T} \Bigg( h_{\$} \sum_{h=1}^{N} \text{used}_{ht} + \frac{m_{\$}}{2} \sum_{h=1}^{N} \sum_{i=1}^{N}  \text{migr}_{iht} \nonumber \\
    &+ th_{\$} \sum_{i=1}^N \text{throt}_{it} + \sum_{h=1}^{N} \sum_{i=1}^{N} \lambda_{iht} (\text{alloc}_{iht} - y_{i(t+1)} \, \text{placed}_{iht}) \Bigg) \label{soft_obj}
\end{align} }
where $\lambda_{iht} \in \R$ are the chosen Lagrange multipliers and $T$ is the optimization horizon. We denote the MILP with the objective \ref{soft_obj} and constraints \ref{c0i} -- \ref{c8ii} as the \textbf{soft MILP}.

Alternatively, we can simply add the soft constraint as a hard constraint to the primary MILP. We call this extended formulation with objective \ref{obj} and constraints \ref{c0i} -- \ref{c8ii}, \ref{c4b} as the \textbf{hard MILP}.






% \subsection{hard MILP Formulation}
% In addition, the \textbf{primary MILP} does not model three facets of the CLOUD packing problem. These are (1) a heuristic that does not allocate more than the actual demand at the next step, (2) variations in arrival and departure of VMs, (3) migration delays. To account for the first unmodeled heuristic we find that adding the following constraint to the \textbf{primary MILP} improves the quality of the solution. The constraint we add states that an VM $i$ (on any host $h$) at time $t$ can only be allocated an amount less than or equal to its upcoming demand ($y_{i(t+1)}$). 
% { \small \begin{align}
%     \;\;\;\; \text{alloc}_{iht} \leq y_{i(t+1)} \; \text{placed}_{iht} \;\;\;\;\;\;\; \forall \; i, \forall \; h, \forall \; t  \label{c4b}
% \end{align} }
% We call this extended formulation the \textbf{hard MILP}. The hosts, migrations and throttled costs of the \textit{primary} and \textit{extended MILP} with a forecasting oracle (\textit{i.e.} perfect forecasts) for different workloads and datasets is tabled in Table \ref{tab:perfect}. We observe that the \textbf{hard MILP} reduce costs by half or more when compared to the \textbf{primary MILP}.  


% % \subsection{soft MILP Formulation}
% % As a soft constraint, inequality \ref{c4b} is traditionally added to the objective as follows.
% % { \small \begin{align}
% %     &\min \; \sum_{t=1}^{T} \Bigg( h_{\$} \sum_{h=1}^{N} \text{used}_{ht} + \frac{m_{\$}}{2} \sum_{h=1}^{N} \sum_{i=1}^{N}  \text{migr}_{iht} \nonumber \\
% %     &+ th_{\$} \sum_{i=1}^N \text{throt}_{it} + \sum_{h=1}^{N} \sum_{i=1}^{N} \lambda_{iht} (\text{alloc}_{iht} - y_{i(t+1)} \, \text{placed}_{iht}) \Bigg) \label{soft_obj}
% % \end{align} }
% % where $\lambda_{iht} \in \R$ are the chosen Lagrange multipliers and $T$ is the optimization horizon. We denote the MILP with the objective \ref{soft_obj} and constraints \ref{c0i} -- \ref{c8ii} as the \textbf{soft MILP}.

% We find that, with a prediction oracle, the sum of the hosts, migrations and throttling costs is significantly lesser in the \textbf{hard MILP} than the \textbf{soft MILP} (see Table \ref{tab:perfect}). We provide a detailed explanation of the same in the Experimental Resulsts section.

% Based on the above observations of hard constraining \ref{c4b} performing the best with the forecasting oracle, we are inspired to extend this to real (and imperfect) forecasts. But, the current predict-and-optimize methods are not suitable for problems where the constraint is parameterized by the forecast. We abstract these formulations below.


% To demonstrate the significant advantage provided by additional constraint \ref{c4b}, we table the costs with and without this constraint when solving the above MILP for different workloads and datasets using a forecasting oracle in Table \ref{tab:perfect} in the Experiments Section. \todo{Anything more?}
% Further, this very same constraint that provides a 2-3x reduction of costs given a perfect oracle, presents a challenge for current predict-and-optimize methods. 

% The output of the forecaster $Y_{it}$ is now a part of the constraints rather than the objective. This leads to the following formulation. 


==> rq1.tex <==












% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[t]
\centering 
\scriptsize 
\begin{tabular}{c|c|c|c|c|c|c}
\hline \hline 
\multicolumn{3}{c|}{Horizon/Methods} & \multicolumn{4}{c}{Datasets}  \\ \cline{4-7} 
\multicolumn{3}{c|}{} &  Mixed10 & HF10 & LF10 & Real10 \\ \hline \hline 

\multirow{6}{*}{H=2} &  two- & soft  & 887.3  & 797.34  & 883.86  & 581.78   \\ 
 &  stage & hard  & \textbf{766.37}  & \textbf{775.1} & \textbf{880.0}  & \textbf{572.19}    \\ \cline{2-7}
 & \multirow{4}{*}{PnO} & SPO  & 739.16  & 744.16  & 734.39   & 173.51   \\
 &  & \cSPO  & \textbf{718.09}  &\textbf{ 707.51}  & \textbf{787.3}  & \textbf{167.09}   \\ % \cline{3-7}
 &  & QPTL  & 1064.69  & 1098.62  & 1050.81 & 669.69   \\
 &   & \cQPTL  & \textbf{920.56} & \textbf{987.25}  & \textbf{1028.8}   & \textbf{592.66}   \\ \hline
\multirow{6}{*}{H=3} & two- & soft  & 1056.12  & 1030.84  & 1023.74 & 556.71   \\
 &  stage & hard & \textbf{933.56}  & \textbf{981.06} & \textbf{905.26} \\ \cline{2-7}
 & \multirow{4}{*}{PnO} & SPO  & 639.34  & 643.51  & 635.82  & 169.65   \\
 &  & \cSPO  & \textbf{635.78}  & \textbf{580.0}  & \textbf{682.6 }& \textbf{157.38}   \\ % \cline{3-7}
 &   & QPTL  & 1034.54  & 1086.15  & 1062.28   & 660.8   \\  
  &  & \cQPTL  & \textbf{837.2}  & \textbf{610.55}  & \textbf{979.89}   & \textbf{634.15}   \\\hline 
\multirow{6}{*}{H=4} & two- & soft  & 1044.19  & 1059.13  & 1041.18   & 554.94   \\ 
 &  stage & hard  & \textbf{955.19}  & \textbf{920.76} & \textbf{941.01}  & \textbf{546.71}    \\ \cline{2-7}
 & \multirow{4}{*}{PnO} & SPO  & 638.74  & 663.69  & 637.17  & 165.42   \\ 
 &  & \cSPO  & \textbf{624.58}  & \textbf{645.55}  & \textbf{549.23} & \textbf{157.2}   \\ % \cline{3-7}
  &  & QPTL  & 1024.89  & 1085.85  & 1095.18  & 660.05   \\ 
  &  & \cQPTL  & \textbf{605.02}  & \textbf{1014.4}  & \textbf{919.19}    & \textbf{627.14}   \\ \hline 
\multirow{6}{*}{H=5} & two- & soft  & 1080.31  & 1073.48  & 1003.66 & 563.5   \\
 &  stage & hard  & \textbf{932.14}  & \textbf{956.12} & \textbf{944.58}  & \textbf{556.27}    \\ \cline{2-7}
 & \multirow{4}{*}{PnO} & SPO  & 638.46  & 642.35  & 601.57     & 216.59   \\
 &  & \cSPO  & \textbf{621.47}  & \textbf{597.53}  & \textbf{533.32}   & \textbf{152.7}   \\ % \cline{3-7} 
  &  & QPTL  & 951.93  & 1063.67  & 1087.92 & 568.73   \\
  &  & \cQPTL  & \textbf{600.81}  & \textbf{631.97}  & \textbf{1075.65} & \textbf{553.37}   \\ 
\hline \hline 
\end{tabular}
\caption{\texttt{(RQ1)} \cQPTL vs QPTL and \cSPO vs SPO in both PnO and PnC.
% Hardened vs LR in PnO. For each horizon and dataset, for a comparison between the hardened extension and the LR extensions, the least regret is made bold. 
%In all cases, the hardened extension beats the LR formulation. 
}
\label{tab:rq1}
\end{table}




==> rq3.tex <==












% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[H]
\centering 
\scriptsize 
\begin{tabular}{c|c|c|c|c|c}
\hline \hline 
\multicolumn{2}{c|}{Methods} & \multicolumn{4}{c}{Datasets}  \\ \cline{3-6} 
\multicolumn{2}{c|}{} &  Mixed10 & HF10 & LF10 & AWS10 \\ \hline \hline 
Heuristics & First Fit & 616.53 & 618.05 & 602.36 & 401.16\\
 & Best Fit  & 602.83 & \underline{611} & \textbf{384.29} & 229.93\\ \hline 
PnC & LRSPO  & 639.16  & 644.16  & 634.39 & \textbf{135.51}  \\
$H=2$ & HASPO  & \textbf{572.49}  & \textbf{535.27}  & 589.48   & \textbf{135.51} \\
 & LRQPTL  & \underline{602.27}  & 1003.58  & \underline{597.5}  & \textbf{135.51}  \\
 & HCQPTL  & 611.27  & 998.35  & 597.5  & \textbf{135.51}  \\
\hline \hline 
\end{tabular}
\caption{RQ3 Heuristics: The lowest regret for each dataset is in bold. The second lowest is underlined. We observe that best fit heuristic is better than PnC itself on Low Frequency data where throttling is little to none.
}
\label{tab:rq3}
\end{table}




==> rq4.tex <==













% \begin{table}[t]

% \end{table}


% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage[normalem]{ulem}
% % \useunder{\uline}{\ul}{}
% \begin{table}[H]
% \centering 
% \scriptsize 
% \begin{tabular}{c|c|c|c}
% \hline \hline 
% \multicolumn{2}{c|}{Methods} & \multicolumn{2}{c}{Migration Delays, Real10 Dataset}  \\ \cline{3-4} 
% \multicolumn{2}{c|}{} &  2 min & 5 min \\ \hline \hline 


% PnO & SPO & 222.59 & 214.95\\
% $H=5$ & \cSPO & 214.06 & \textbf{167.33}\\
%  & QPTL & 520.64 & 481.56\\
%  & \cQPTL & 585.54 & 588.58\\ \hline 
% PnC & SPO & \textbf{138.51} & \underline{173.51}\\
% $H=2$ & \cSPO & \textbf{138.51} & 320.84\\
%  & QPTL & \textbf{138.51} & \underline{173.51}\\
%  & \cQPTL & \textbf{138.51} & 369.95\\
 
% \hline \hline 
% \end{tabular}
% \caption{RQ4 Migration Delay: Even under significantly different simulation conditions with migration delays, PnC can perform well without observing any migration delayed data at training time.
% }
% \label{tab:rq4_migr}
% \end{table}



==> sine_data_table_5.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage[normalem]{ulem}
% % \useunder{\uline}{\ul}{}
% \begin{table*}[]
% \centering 
% \begin{tabular}{llll|lllllll}
% \hline
% \multicolumn{3}{l}{Workload}                                                               &                                                      & \multicolumn{5}{c|}{Forecast Horizon = 5, Simulation Time = 25}                                   & \multicolumn{2}{l}{Heuristics; No Forecast} \\ \hline
% Dataset & N  & Arrival                                                                     & \begin{tabular}[c]{@{}l@{}}Migr\\ Delay\end{tabular} & Two-stage & HC-QPTL & HA-SPO    & LR-QPTL      & LR-SPO            & First Fit               & Best Fit          \\ \hline
% Mixed   & 5  & \multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}All \\ at \\ start\end{tabular}} & \multirow{6}{*}{None}                                & -225.9    &     & &  {\ul -188.6} & \textbf{-180.29} &           -209.3                  & -205.7            \\
% Mixed   & 10 &                                                                             &                                                      &           &           & &             &                  &                                   &                   \\
% Spiky   & 5  &                                                                             &                                                      & -209.7    &     & & {\ul -172.2} & \textbf{-168.86} &           -186.9                  & -190              \\
% Spiky   & 10 &                                                                             &                                                      &           & \textbf{} & & {\ul }       &                  &                                   &                   \\
% Smooth  & 5  &                                                                             &                                                      & -200.2    &       & & {\ul -176}   & {\ul -176}       &           \textbf{-144}           & -192              \\
% Smooth  & 10 &                                                                             &                                                      &           & \textbf{} & & \textbf{}    &                  &                                   &                   \\ \hline
% \end{tabular}
% \caption{Synthetic Dataset Performance of various policies (forecast horizon of 5) and heuristics. The lowest neagtive reward is made bold and the second lowest is underlined.}
% \label{tab:sine_data_3}
% \end{table*}
